ToDA: Target-oriented Diffusion Attacker against Recommendation System

Recommendation systems (RS) have become indispensable tools for web services to address information overload, thus enhancing user experiences and bolstering platforms' revenues. However, with their increasing ubiquity, security concerns have also emerged. As the public accessibility of RS, they are susceptible to specific malicious attacks where adversaries can manipulate user profiles, leading to biased recommendations. Recent research often integrates additional modules using generative models to craft these deceptive user profiles, ensuring them are imperceptible while causing the intended harm. Albeit their efficacy, these models face challenges of unstable training and the exploration-exploitation dilemma, which can lead to suboptimal results. In this paper, we pioneer to investigate the potential of diffusion models (DMs), for shilling attacks. Specifically, we propose a novel Target-oriented Diffusion Attack model (ToDA). It incorporates a pre-trained autoencoder that transforms user profiles into a high dimensional space, paired with a Latent Diffusion Attacker (LDA)-the core component of ToDA. LDA introduces noise into the profiles within this latent space, adeptly steering the approximation towards targeted items through cross-attention mechanisms. The global horizon, implemented by a bipartite graph, is involved in LDA and derived from the encoded user profile feature. This makes LDA possible to extend the generation outwards the on-processing user feature itself, and bridges the gap between diffused user features and target item features. Extensive experiments compared to several SOTA baselines demonstrate ToDA's effectiveness. Specific studies exploit the elaborative design of ToDA and underscore the potency of advanced generative models in such contexts.

==> sections/2-Related.tex <==
\section{Related Work}
This section organizes the related work into two branches: shilling attacks on recommendation system and the use of diffusion models across various disciplines.


\subsection{Shilling Attacks on Recommendation System}

Recommendation system is essential for curating and delivering personalized content across various digital platforms. Significant advancements have been achieved through methods such as Bayesian Personalized Ranking~\cite{BPR} and Neural Collaborative Filtering~\cite{NCF}. Furthermore, graph-based recommendation techniques~\cite{LightGCN}, along with self-supervised learning approaches~\cite{SGL, SLMRec}, have propelled the field forward. However, these developments also heighten these systems' vulnerability to attacks. 
Much effort has been devoted to developing robust recommendations to counteract potential threats. ~\cite{FNCF} proposes a defensive strategy that employs a noise layer and intermediate outputs from a teacher model. ~\cite{AMR} employs adversarial learning to fortify systems against these perturbations. EliMRec~\cite{EliMRec} uses causal inference and counterfactual reasoning to detect and eliminate such biases.

Despite the boosting of robustness, recommendation system is still under the threat of some specific attacks, \ie shilling attacks, where malicious attackers introduce fake user data/profiles into the training datasets of Recommendation system, potentially compromising their integrity and effectiveness ~\cite{TrustworthyRS}. Some heuristic-based methods craft the user profiles manually~\cite{shillingAttack}, for instance, executing a strategy where attackers enhance the authenticity of their ratings by rating non-target items based on average system ratings, while simultaneously rating target items at extremes, termed average attack.
Afterwards, optimization-based methods~\cite{PAGR,RevAttack,DLAttack, fang2020influence} formulate the attack task as learnable objectives, leading to an automatic generation of fake users.
Wherein, Zhang \etal use a reference matrix from a surrogate model to capture key item relationships, enabling attackers to craft fake user profiles that effectively distort these relationships~\cite{ReverseAttack}. 
Zhang \etal incorporates a bi-level optimization framework and a reverse learning process to bypass privacy safeguards and disrupt the recommendation system~\cite{RAPU-R}.
Li \etal formulates data poisoning attacks as a bi-level optimization problem, leveraging the interconnectivity of these domains to launch data poisoning attacks~\cite{DPAF}.

Recent studies have increasingly pivoted towards leveraging generative models to orchestrate more sophisticated attack strategies. 
Zeng \etal proposes to employ self-supervised learning techniques on publicly available data to improve the attack efficacy over traditional methods~\cite{PCAttack}. 
Similarly, there are several methods that utilize Generative Adversarial Networks (GANs) as generative models, such as GAN-based approaches ~\cite{TriAttack, GSA-GAN, AUSH, LegUP, GSPAttack}, as well as methods based on Reinforcement Learning (RL)~\cite{ARG, TDP-CP, KGAttack, CopyAttack, LOKI, Poisonrec}, which operate in an autoregressive manner. 
These methods build upon the strategies mentioned earlier but introduce generative models to create fake interactions and user profiles, replacing traditional strategies and heuristic methods. Benefiting from  generative capabilities, these methods demonstrate exceptional attack capability while ensuring imperceptibility compared to the previously mentioned approaches. However, to achieve malicious objectives, an additional attack module is often incorporated, either by utilizing influence functions~\cite{TriAttack} or by formulating additional optimization objectives~\cite{LegUP}. 
Despite these advancements, more compatible generative models, such as Diffusion Models (DMs), remain unexplored, lacking a consistent way to achieve both imperceptibility and harmfulness.
We introduce a new generative paradigm for the future shilling attacks, ToDA, mitigating the learning dilemma and inflexibility of recent GAN- and RL-based methods. We go beyond the simple utilization of DMs to achieve light-weight and malicious intent.


\subsection{Diffusion Models}
Diffusion models (DMs) operate by decomposing the data formation process into a sequential application of denoising autoencoders. 
Consequently, DMs have been widely used to generate high-quality, controllable synthetic data~\cite{DMs_Survey}. 
Simultaneously, DMs are emerging as a robust alternative to GANs across various applications~\cite{DM_ImageSynthesis, DM_TopologyOptim, DM_ImageClass}.

Over the years, a range of diffusion-based generative models have been introduced, featuring core similarities but distinct implementations. 
A notable example is Denoising Diffusion Probabilistic Models (DDPMs)~\cite{DDPM}, which operate by training on a weighted variational bound designed according to a novel connection between diffusion probabilistic models and denoising score matching with Langevin dynamics.
Despite initially being extensively researched and used in the field of image generation, DMs find extensive utility across diverse domains beyond vision-relevant tasks~\cite{DMs_vision_survey}, such as graph~\cite{DMs_graphSurvey} and natural language processing~\cite{Diffuser, Diffuseq}.

Recently, DMs have been leveraged for more complex tasks, demonstrating superior performance in previously unexplored domains. 
Specifically, in the field of recommendation system, DiffRec learns the generative process in a denoising manner. To retain personalized information in user interactions, DiffRec reduces the added noise and avoids corrupting users' interactions into pure noise, unlike in image synthesis~\cite{DiffRec}.
Additionally, DiffuRec represents item embeddings as distributions, corrupts the target item embedding into a Gaussian distribution via noise addition, and, based on the user's historical interaction behaviors, reverses a Gaussian noise into the target item representation, followed by a rounding operation for target item prediction~\cite{DiffuRec}.
Furthermore, in the domain of adversarial attacks, DMs contribute to the mitigation of sample perturbations by first diffusing the sample with a small amount of noise following a forward diffusion process, and then recovering the clean image through a reverse generative process~\cite{DM_purification}. DMs are also used in DiffAttack, which crafts perturbations in the latent space of DMs. By combining these perturbations with well-designed content-preserving structures, human-insensitive perturbations embedded with semantic clues can be generated~\cite{DiffAttack}. Additionally, DMs enhance model robustness~\cite{DM-Improves-AT, DensePure}.

In efforts to guide generated results, substantial strides have been made in text-image generation~\cite{LDM, ControlNet, Diffusionclip}, rendering the process more controllable. Distinct from previous work, our research elucidates the potential and application of using DMs to conduct shilling attacks, taking into account domain conflicts and controllable attack targets.
Moreover, we primarily alleviate the computational burdgen of conventional DMs, and simultaneously enpower DMs with global horizon via GCN techniques to achieve shilling attacks. From our theoretical and empirical analysis, our adaptions of DMs are both reasonable and effective. 

